SoK: A Stratified Approach to Blockchain Decentralization

Decentralization has been touted as the principal security advantage which propelled blockchain systems at the forefront of developments in the financial technology space. Its exact semantics nevertheless remain highly contested and ambiguous, with proponents and critics disagreeing widely on the level of decentralization offered by existing systems. To address this, we put forth a systematization of the current landscape with respect to decentralization and we derive a methodology that can help direct future research towards defining and measuring decentralization. Our approach dissects blockchain systems into multiple layers, or strata, each possibly encapsulating multiple categories, and it enables a unified method for measuring decentralization in each one. Our layers are (1) hardware, (2) software, (3) network, (4) consensus, (5) economics ("tokenomics"), (6) client API, (7) governance, and (8) geography. Armed with this stratification, we examine for each layer which pertinent properties of distributed ledgers (safety, liveness, privacy, stability) can be at risk due to centralization and in what way. We also introduce a practical test, the "Minimum Decentralization Test" which can provide quick insights about the decentralization state of a blockchain system. To demonstrate how our stratified methodology can be used in practice, we apply it fully (layer by layer) to Bitcoin, and we provide examples of systems which comprise one or more "problematic" layers that cause them to fail the MDT. Our work highlights the challenges in measuring and achieving decentralization, and suggests various potential directions where future research is needed.

==> sections/case_studies.tex <==
\section{Case Studies}

We now briefly present and compare two indicative case studies, Bitcoin and
Solana.\footnote{Bitcoin
data collected from
\href{https://www.asicminervalue.com/}{ASICMinerValue},
\href{https://bitnodes.io}{BitNodes},
\href{https://miningpoolstats.stream/bitcoin}{MiningPoolStats}.
Solana data collected from the
\href{https://docs.solana.com/cluster/overview}{Solana Docs},
\href{https://www.validators.app/data-centers?locale=en\&network=mainnet\&sort\_by=asn}{validators.app},
\href{https://solanabeach.io/}{SolanaBeach}. 
Data on both systems collected from \href{https://www.coincarp.com/}{CoinCarp},
\href{https://coinmarketcap.com}{CoinMarketCap},
\href{https://nomics.com}{nomics}.
[August $2022$]} 
The goal of this section is to illustrate how our methodology can be used to
estimate and compare the decentralization levels of real-world systems. We note
that the following paragraphs offer qualitative results only; measuring each
resource's distribution, in a way that enables quantitative comparisons,
is out of scope for the present investigation. 
We also note that no reliable data could be found for either system regarding 
light clients and governance, so no comparison can be conducted for these 
systems on these layers.

\subsubsection*{Hardware}

\paragraph{Bitcoin}
No concrete data could be found on the distribution of hashing power across PoW
mining products. The market offers hundreds of efficient (ASIC) products, while
mining can also be conducted on generic hardware (\eg GPUs). Interestingly,
only few ASICs are profitable, so, unless the token's price increases, mining
should be expected to concentrate around these products. In addition, the
market is already predominantly centralized around only $4$ ASIC
manufacturers~\cite{tokeninsight-2}.

\paragraph{Solana}
Solana's full nodes are predominantly hosted on cloud services, something that further
complicates the evaluation of its hardware layer \wrt specific products and their
manufacturers. %, (\eg the actual CPUs that operate the virtual machines offered by the cloud providers.
%
Nonetheless, in terms of hosting, Solana in highly
centralized, with more than $50$\% and $66$\% of its stake hosted by $3$ and
$5$ providers respectively.

\paragraph{Comparison}
In both systems centralization around a handful of hardware providers is 
present, with Solana notably relying on cloud services and virtualized hardware. 


\subsubsection*{Software}

\paragraph{Bitcoin}
In terms of full node software, almost all nodes ($99.15$\%) run Bitcoin Core.
Therefore, Bitcoin is completely centralized around --- different releases ---
of this product. However, the development of Bitcoin Core is somewhat
decentralized, with over $100$ monthly active core developers~\cite{devtrends}.
%
Regarding the distribution of tokens across wallets, no data could be found.

\paragraph{Solana}
Solana is supported by a single full node product of the Solana
Foundation. This product is maintained by approx. $30$ monthly active core
developers~\cite{devtrends}.

\paragraph{Comparison}
Although both systems depend --- in effect --- completely on a single software
product, Bitcoin's development is significantly more decentralized than
Solana's, with a large set of independent monthly contributors.
%
Instead, Solana's development appears to be covered by a single entity. 

\subsubsection*{Network}

\paragraph{Bitcoin}
Regarding peer discovery, Bitcoin Core permits $8$ outgoing and $125$ incoming
connections, chosen randomly from known identities and/or hardcoded DNS seeds.
Most Bitcoin nodes communicate over Tor, thus complicating topology analyses;
Nonetheless, it is estimated that the network is fairly evenly spread across
multiple Autonomous Systems, thus presenting a high degree of
decentralization.

\paragraph{Solana}
Solana mostly uses UDP, therefore connections are not actively maintained by the underlying
communication protocol; 
instead nodes join ``clusters'' via hardcoded entry nodes. In terms of
topology, Solana is highly centralized, as a vast majority of nodes is
hosted by a handful of cloud providers.

\paragraph{Comparison}
%Bitcoin uses TCP, as opposed to Solana's UDP, so it is unclear how to compare
%the two in terms of peer discovery. 
In terms of network topology 
Bitcoin demonstrates a significant level of decentralization, whereas Solana
sits on the other --- far --- end of the spectrum.

\subsubsection*{Consensus}

\paragraph{Bitcoin}
On the consensus layer, Bitcoin presents mixed results regarding
decentralization. On the one hand, hashing power is distributed across
thousands (possibly millions) of machines; although no concrete data could be
found, folklore evidence suggests that these machines are owned by a highly
diverse set of users. However, Bitcoin also observes high levels of
centralization around pools, \ie \wrt block formation and the input to the PoW
module; specifically, at the time of writing, 
$4$ pools control more than $60$\% of the whole network's
mining power.

\paragraph{Solana}
Solana relies on PoS for Sybil resilience. Therefore, the distribution of
staking power is equivalent to the wealth distribution of tokens to
stakeholders (see below).
%
Solana stakeholders typically delegate their staking rights to validators. As
of $2022$, $29$ validators control more than $33$\% of all participating stake,
thus being able to violate the system's liveness if colluding, $54$ validators
control a stake majority, and $128$ control more than $66$\%, thus being able
to possibly violate safety via a fork.

\paragraph{Comparison}
The lack of data makes it difficult to compare the two systems \wrt the
distribution of the resource (hashing and staking power respectively) across
their owners. On one hand,  Solana demonstrates a
 higher degree of decentralization than Bitcoin at the pooled resource level,
 \ie the resource distribution that arises after parties  
 organize themselves in collaborative entities.  This being said, Bitcoin mining pools
 have a more collaborative nature (pool members are active participants in terms
 of contributing to the total mining power by continuously running the pool protocol), while
 stake pool members in the case of Solana are more passive in the sense they 
 do not actively execute a collaborative protocol for processing blocks. 
 

\subsubsection*{Tokenomics}

\paragraph{Bitcoin}
At its onset, no Bitcoin tokens existed; instead, they were generated and
allocated as the system progressed. However, early participants were
disproportionately favored, with half of all tokens created within the first
two years of its existence, when consensus participation was sparse and by only
a few parties. As the system progressed and more transactions occurred, the
tokens were distributed more widely, albeit wealth is still significantly
centralized, compared to real-world economies (cf. Table~\ref{tab:gini}).
Specifically, approx. $43$M addresses own some amount of tokens, but the top
$100$ addresses control $14.01$\% of all wealth. Nonetheless, tokens are traded
on more than $100$ marketplaces at volumes of approx. \$$53$B.

\paragraph{Solana}
Solana tokens were mostly allocated to prospective users before the system's launch. Of the
initial investors, $48$\% of tokens were held by ``insiders'', including
developers and venture capital, a further $33$\% were put aside for future
development, while the rest were allocated via a public
offering~\cite{solanaDecentralized}. As the system evolved, token ownership
continued being centralized, with $100$ of approx. $9$M addresses controlling
$31$\% of all tokens. Nonetheless, Solana tokens are available in $75$ exchanges
at volumes of approx. \$$1$B.

\paragraph{Comparison}
Evidently, Solana is significantly more centralized than Bitcoin \wrt token
ownership, both at the systems' onset and as they evolved. In terms of
secondary markets, although both tokens are available in tens of exchanges,
Bitcoin's both trading volume and, more importantly, trading pairs are
significantly higher than Solana's ($9622$ pairs for Bitcoin to Solana's
$383$), indicating a much more liquid market for Bitcoin.


\subsubsection*{Geography}

\paragraph{Bitcoin}
In $2019$, Bitcoin mining hardware was mostly located in China (and 
particularly Sichuan) and the US (mostly Washington and New 
York)~\cite{bendiksen2019bitcoin,kohler2019life}. Interestingly, at that time 
---and until the ban of mining in China in 2021--- the mining pools located in 
China accounted for  $\sim 70\%$ of the total hashrate~\cite{stoll2019carbon,cbecimining}. 
In $2022$, a large fraction of the nodes communicates over 
Tor,\footnote{$46.5$\% of Bitcoin's nodes operate over Tor. 
[\href{https://bitnodes.io/dashboard/}{bitnodes}; August $2022$]} which makes
analyzing the network's topology particularly hard. Nonetheless, Bitcoin
miners, although fairly well distributed with a presence in 95 different 
countries, tend to cluster in certain areas.
More than $\frac{1}{3}$ of mining is located in the USA, with Kazakhstan and
Russia following with $18$\% and $11$\% respectively~\cite{cbecimining}.
In terms of full nodes (which may not participate in mining), USA and Germany
see roughly equivalent shares, with other countries hosting far fewer nodes 
(see also Table \ref{tab:countries}), although still a majority communicates 
anonymously.

\paragraph{Solana}
Solana validators and RPC nodes appear to operate from more than 25 different 
countries. However, there is significant centralization in some countries., 
with more than a quarter of the $3,455$ full nodes based in the US and 
another fifth in Germany.\footnote{Source: 
\href{https://solanabeach.io/}{solanabeach.io}, August 2022} 

\paragraph{Comparison}
Bitcoin's full nodes are spread across many more countries than Solana's, but 
both systems exhibit centralization tendencies towards certain countries. After 
the ban of mining in China in 2021, Bitcoin appears to be the most 
decentralized of the two. 

\subsubsection*{Summary}

Analyzed in six of our eight layers (Hardware, Software, Network, 
Consensus, Tokenomics, Geography), Bitcoin is clearly ahead in four of them 
(software, network, tokenomics, geography), with the remaining two either 
being too close and incomparable to decide (hardware), or Solana having some potential edge (consensus). 

In terms of the Minimum Decentralization Test (cf. Definition~\ref{def:mdt}),
we can say that Bitcoin passes the test while Solana does not, due to 
a single legal entity being responsible for development in the software layer. 


==> sections/dimensions.tex <==
\medskip
\textbf{Dimensions of Decentralization and Paper 
Structure}\label{sec:dimensions}
We identify $8$ layers in a distributed ledger where decentralization must be examined:
\begin{inparaenum}[(1)]
    \item Hardware;
    \item Software;
    \item Network;
    \item Consensus;
    \item Economics (``Tokenomics'');
    \item Client API;
    \item Governance;
    \item Geography.
\end{inparaenum}
Each is divided into sub-categories and analyzed using the framework outlined
above.
Specifically, 
%
Section~\ref{sec:hardware} looks into the hardware and diversity in
manufacturers of mining equipment and cloud hosting.  
% 
Section~\ref{sec:software} focuses on the major types of relevant software, 
that realize participation and asset management,
and the diversity of software products and
development teams.
% 
Section~\ref{sec:p2p} considers the network over which the nodes
communicate and evaluates decentralization on both a microscopic level, \wrt a
specific node's network access, and a
macroscopic level, \wrt the overall network's topology.
% 
Section~\ref{sec:consensus} explores the consensus mechanism and categorizes
systems based on the mode of participation they allow.
%
Section~\ref{sec:wealth} focuses on the economics of blockchain systems and
evaluates the hazards of a centralized initial token distribution,
subsequent control of the ledger's native tokens by few investors, and
centralization in few secondary markets.
%
Section~\ref{sec:clients} brings attention to the services that are 
often used as an interface to a blockchain, whose enhanced efficiency and 
scalability may come at the expense of security and decentralization.
%
Sections~\ref{sec:governance} and~\ref{sec:geography} explore
multi-layer dimensions; Section~\ref{sec:governance} examines governance, \ie how 
peers propose and decide on system improvements and funding allocation, while 
Section~\ref{sec:geography} delves into the geographic and jurisdictional distribution 
of blockchain systems.
%
Section~\ref{sec:case-studies} presents case studies, where all of the above 
decentralization dimensions are evaluated for a specific system, 
\ifshort
Bitcoin,\footnote{Appendix 
\ref{sec:evaluations} provides per-layer evaluations that include additional 
systems.} and several other systems are shown to fail the MDT.
\else
Bitcoin and enable us to apply the MDT.
\fi
Finally, Section~\ref{sec:conclusion} enhances the discussion 
with various possible research directions.


==> sections/overview.tex <==
\begin{table*}
    \centering
    \begin{tabular}{ccccp{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}}

        &
        &
        &
        & \multicolumn{4}{c}{\textbf{Property Hazards}}
        \\
          \textbf{Layer}
        & \textbf{Subcategory}
        & \textbf{Resources}
        & \textbf{Relevant Parties}
        & \rotatebox{45}{\emph{Safety}}
        & \rotatebox{45}{\emph{Liveness}}
        & \rotatebox{45}{\emph{Privacy}}
        & \rotatebox{45}{\emph{Stability}}
        \\
        \specialrule{1.6pt}{1pt}{1pt}
        \\

        \multirow{5}{*}{\textbf{Hardware}}
        & Proof-of-Work
        & Hashing power
        & \begin{tabular}[c]{@{}c@{}} Manufacturers of \\ mining hardware 
        \end{tabular}
        & \pie{360}
        & \pie{360}
        & \pie{0}
        & \pie{90}
        \\
        \\
        \cdashline{2-8}
        \\


        & Proof-of-Stake
        & Stake
        & Hosting providers
        & \pie{360}
        & \pie{360}
        & \pie{360}
        & \pie{90}
        \\
        \hline
        \\

        \ifshort
        \multirow{5}{*}{\textbf{Software}}
        \else
        \fi
        & Protocol participation
        & \begin{tabular}[c]{@{}c@{}} 1) Hashing/Staking power \\ 2) Full nodes 
        \end{tabular}
        & \begin{tabular}[c]{@{}c@{}} Developers of \\ full node software 
        \end{tabular}
        & \pie{360}
        & \pie{360}
        & \pie{90}
        & \pie{360}
        \\
        \\
        \cdashline{2-8}
        \\


        \ifshort
        \else
        \textbf{Software}
        \fi
        & Asset management
        & Tokens
        & \begin{tabular}[c]{@{}c@{}} Developers of \\ wallet software 
        \end{tabular}
        & \pie{0}
        & \pie{360}
        & \pie{270}
        & \pie{360}
        \ifshort
        \\
        \hline
        \\
        \else
        \\
        \\
        \cdashline{2-8}
        \\
        \fi


        \ifshort
        \else
        & Testing
        & Testnets
        & Development teams
        & \pie{90}
        & \pie{90}
        & \pie{90}
        & \pie{90}
        \\
        \hline
        \\
        \fi

        \multirow{4}{*}{\textbf{Network}}
        & Peer discovery
        & (Single node's) Connections
        & Owners of peers
        & \pie{360}
        & \pie{360}
        & \pie{90}
        & \pie{0}
        \\
        \\
        \cdashline{2-8}
        \\


        & Topology
        & Bridges between components
        & Owners of bridges
        & \pie{180}
        & \pie{180}
        & \pie{90}
        & \pie{0}
        \\
        \hline
        \\

        \multirow{5}{*}{\textbf{Consensus}}
        & Direct Participation
        & \begin{tabular}[c]{@{}c@{}} 1) Hashing/Staking power \\ 2) Block content \end{tabular}
        & \begin{tabular}[c]{@{}c@{}} Owners of \\ participation nodes 
        \end{tabular}
        & \pie{360}
        & \pie{360}
        & \pie{90}
        & \pie{270}
        \\
        \\
        \cdashline{2-8}
        \\


        & Representative Participation
        & Validator identities
        & \begin{tabular}[c]{@{}c@{}} Owners of \\ validator nodes \end{tabular}
        & \pie{360}
        & \pie{360}
        & \pie{0}
        & \pie{270}
        \\
        \hline
        \\

        & Initial token distribution
        & Tokens (during bootstrapping)
        & Token holders
        & \pie{90}
        & \pie{90}
        & \pie{0}
        & \pie{360}
        \\
        \\
        \cdashline{2-8}
        \\


        \begin{tabular}[c]{@{}c@{}} \textbf{Cryptocurrency} \\ \textbf{Economics} \end{tabular}
        & Token ownership
        & Tokens
        & \begin{tabular}[c]{@{}c@{}} 1) Addresses \\ 2) Key-holding parties \\ 3) Legal stakeholders \end{tabular}
        & \pie{90}
        & \pie{90}
        & \pie{0}
        & \pie{360}
        \\
        \\
        \cdashline{2-8}
        \\


        & Secondary markets
        & Liquidity (tokens on sale)
        & \begin{tabular}[c]{@{}c@{}} 1) Exchanges \\ 2) Trading pairs \end{tabular}
        & \pie{90}
        & \pie{90}
        & \pie{360}
        & \pie{360}
        \\
        \hline
        \\

        \textbf{Light Clients}
        &
        & \begin{tabular}[c]{@{}c@{}} 1) Tokens of light wallets \\ 2) Light nodes \end{tabular}
        & Owners of full nodes
        & \pie{360}
        & \pie{360}
        & \pie{360}
        & \pie{270}
        \\
        \midrule[1pt]
        \\

        \multirow{4}{*}{\textbf{Governance}}
        & Improvements \& conflict resolution
        & Decision-making power
        & All parties in ecosystem
        & \pie{90}
        & \pie{90}
        & \pie{0}
        & \pie{360}
        \\
        \\
        \cdashline{2-8}
        \\


        & Development funding
        & Capital
        & Development teams
        & \pie{0}
        & \pie{0}
        & \pie{0}
        & \pie{360}
        \\
        \hline
        \\

        \multirow{4}{*}{\textbf{Geography}}
        & Physical safety
        & All resources above
        & Regions
        & \pie{180}
        & \pie{180}
        & \pie{0}
        & \pie{90}
        \\
        \\
        \cdashline{2-8}
        \\


        & Legal compliance
        & All resources above
        & Jurisdictions
        & \pie{90}
        & \pie{90}
        & \pie{360}
        & \pie{360}
        \\
        \hline
        \\
    \end{tabular}
    \caption{
        Overview of blockchain decentralization layers. \\
        \normalfont{
            Property hazards come at different degrees: 
            i) black circle: direct hazards;
            ii) $270^{\circ}$ : implementation-depending hazards;
            iii) $180^{\circ}$: either/or scenario (\eg either safety or liveness violated);
            iv) $90^{\circ}$: indirect hazards;
            v) white circle: no hazards.
        }
    }
    \label{tab:summary}
\end{table*}


